Defending Against Repetitive Backdoor Attacks on Semi-supervised Learning through Lens of Rate-Distortion-Perception Trade-off

Semi-supervised learning (SSL) has achieved remarkable performance with a small fraction of labeled data by leveraging vast amounts of unlabeled data from the Internet. However, this large pool of untrusted data is extremely vulnerable to data poisoning, leading to potential backdoor attacks. Current backdoor defenses are not yet effective against such a vulnerability in SSL. In this study, we propose a novel method, Unlabeled Data Purification (UPure), to disrupt the association between trigger patterns and target classes by introducing perturbations in the frequency domain. By leveraging the Rate-Distortion-Perception (RDP) trade-off, we further identify the frequency band, where the perturbations are added, and justify this selection. Notably, UPure purifies poisoned unlabeled data without the need of extra clean labeled data. Extensive experiments on four benchmark datasets and five SSL algorithms demonstrate that UPure effectively reduces the attack success rate from 99.78% to 0% while maintaining model accuracy. Code is available here: \url{https://github.com/chengyi-chris/UPure}.

==> tables/tab-abl-diff-area.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[!ht]
\begin{center}
\caption{Effects on Different areas}
\label{tab:abl-diff-area}
\scalebox{0.9}{
\begin{tabular}{clllllll}
\toprule
%\hline\noalign{\smallskip}
\multirow{2}{*}{Size of region} & \multicolumn{3}{c}{CIFAR10} & &\multicolumn{3}{c}{SVHN} \\
\cmidrule{2-4} \cmidrule{6-8}
& \multicolumn{1}{c}{BA} & ASR &PSNR & &\multicolumn{1}{c}{BA} & ASR &PSNR \\
\midrule
No defense &92.80&97.54&-&&97.61&98.76&-\\
\midrule
4x4  &91.67&98.41&49.24&&96.71&99.64&50.51\\
8x8 &92.15&96.97&46.91&&96.88&98.93&49.64\\
16x16 &91.05&0.00&45.43&&96.49&0.00&48.75\\
24x24 &90.57&0.00&43.07&&95.84&0.00&47.02\\
\bottomrule
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

==> tables/tab-abl-rate.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[!ht]
\begin{center}
\caption{Effects on Poisoning Rates}
\label{tab:abl-poison-rate}
\scalebox{0.9}{
\begin{tabular}{clllll}
\toprule
%\hline\noalign{\smallskip}
\multirow{2}{*}{Poisoning Rate(\%)} & \multicolumn{2}{c}{Attack} & &\multicolumn{2}{c}{Our Defense} \\
\cmidrule{2-3} \cmidrule{5-6}
& \multicolumn{1}{c}{BA} & ASR& &\multicolumn{1}{c}{BA} & ASR \\
\midrule
0.15 &92.76&71.16&&91.35&0.00\\
0.2 &92.86&96.91&&91.05&0.00\\
0.3 &93.18&98.20&&91.90&0.00\\
0.4 &92.27&98.76&&92.18&0.00\\
0.5 &90.62&98.52&&90.42&0.00\\
\bottomrule
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

==> tables/table_template.tex <==

\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Font sizes of headings. Table captions should always be positioned {\it above} the tables. The final sentence of a table caption should end without a full stop}
\label{table:headings}
\begin{tabular}{lll}
\hline\noalign{\smallskip}
Heading level & Example & Font size and style\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
Title (centered)  & {\Large \bf Lecture Notes \dots} & 14 point, bold\\
1st-level heading & {\large \bf 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold
\\
4th-level heading & {\it Remark.} Text follows \dots & 10 point,
italic\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
